Computed Tomography Image Enhancement using 3D Convolutional Neural Network

Computed tomography (CT) is increasingly being used for cancer screening, such as early detection of lung cancer. However, CT studies have varying pixel spacing due to differences in acquisition parameters. Thick slice CTs have lower resolution, hindering tasks such as nodule characterization during computer-aided detection due to partial volume effect. In this study, we propose a novel 3D enhancement convolutional neural network (3DECNN) to improve the spatial resolution of CT studies that were acquired using lower resolution/slice thicknesses to higher resolutions. Using a subset of the LIDC dataset consisting of 20,672 CT slices from 100 scans, we simulated lower resolution/thick section scans then attempted to reconstruct the original images using our 3DECNN network. A significant improvement in PSNR (29.3087dB vs. 28.8769dB, p-value < 2.2e-16) and SSIM (0.8529dB vs. 0.8449dB, p-value < 2.2e-16) compared to other state-of-art deep learning methods is observed.

==> source files/0_abs.tex <==
\begin{abstract}
Computed tomography (CT) is increasingly being used for cancer screening, such as early detection of lung cancer. However, CT studies have varying pixel spacing due to differences in acquisition parameters. Thick slice CTs have lower resolution, hindering tasks such as nodule characterization during computer-aided detection due to partial volume effect. In this study, we propose a novel 3D enhancement convolutional neural network (3DECNN) to improve the spatial resolution of CT studies that were acquired using lower resolution/slice thicknesses to higher resolutions.  Using a subset of the LIDC dataset consisting of 20,672 CT slices from 100 scans, we simulated lower resolution/thick section scans then attempted to reconstruct the original images using our 3DECNN network. A significant improvement in PSNR (29.3087dB vs. 28.8769dB, p-value $< 2.2e-16$) and SSIM (0.8529dB vs. 0.8449dB, p-value $< 2.2e-16$) compared to other state-of-art deep learning methods is observed. 

% This method could be used to overcome inherent partial volume effects that reduce the accuracy of quantitative measurements. With the same 3DECNN architecture, it also paves the way for other CT image enhancement tasks, such as generating high-dose-like CT from low-dose scans.


% Traditional super resolution methods like bicubic interpolation generate many artifacts, including jagged edges and blurring. Unlike existing work in SR enhancement, which has been demonstrated on 2D natural images or chest radiographs, CT images are volumetric with strong correlation between slices. {\color{red} {(paragraph3:)} } Using a large public dataset of CT images, we demonstrate how our 3DSR-CNN architecture achieves better peak signal-to-noise ratio and structure similarity index compared to existing state-of-the-art SR work. {\color{red} {(paragraph4:)} } We demonstrate that: 1) utilizing a 3D approach that makes use of positional correlations between CT slices can improve image quality and 2) 3DSR-CNN approaches can potentially be used overcome inherent partial volume effect that reduce the accuracy of quantitative measurements. 

\keywords{super resolution, computed tomography, medical imaging, convolutional neural network, image enhancement, deep learning}
\end{abstract}

==> source files/1_intro.tex <==
\section{Introduction}

%{\color{red} {change this paragraph to reflect the resolution change rather than dose. You could reference the abstract}} 

Computed tomography (CT) is a widely used screening and diagnostic tool that provides detailed anatomical information on patients. Its ability to resolve small objects, such as nodules that are 1-30 mm in size, makes the modality indispensable in performing tasks such as lung cancer screening and colonography. However, the variation in image resolution of CT screening due to differences in radiation dose and slice thickness hinders the radiologist's ability to discern subtle suspicious findings. Thus, it is highly desirable to develop an approach that enhances lower resolution CT scans by increasing the detail and sharpness of borders to mimic higher resolution acquisitions~\cite{SRmedical}. %Recently, the high resolution CT (HRCT) is ideal because it is capable of resolving very small objects with minimal noise, making it easier for radiologists to detect\cite{HRCT}. However, HRCT imparts a high radiation dose on patients. In patients with emphysema or chronic obstructive pulmonary disease, patients have difficulty holding their breath for the required scanning time. It is highly desirable to get high resolution images using (ultra) low-dose computed tomography (LDCT), which utilizes minimal radiation dose\cite{HRCT2} and shorter scan times. We investigate how LDCT studies can potentially be upsampled to match HRCT images using super resolution image reconstruction\cite{SRmedical}. 

%Super resolution (SR)\cite{SR} is a class of techniques that increase the resolution of an imaging system\cite{SRoverview}. SR can be divided into two categories, multiple-frame SR and single-frame SR. Multiple-frame SR uses the sub-pixel shifts between multiple low resolution images of the same scene and create a higher resolution image. Single-frame SR attempts to magnify the image without introducing blur. These methods use other parts of the low resolution images, or other unrelated images, to provide an informed estimate of what the high resolution image should look like.

%The conventional linear methods for SR enhancement like bilinear and bicubic interpolation generate blurring and jagged artifacts. An alternative approach is example-based, which learns the mapping function from low-resolution (LR) and high-resolution (HR) pairs. The sparse-coding-based (SC) method is one of the representative example-based SR methods\cite{sparse}. Junko \emph{et al}. \cite{sparse1} has applied the sparse-coding-based SR method to CT imaging. Nowadays, convolutional neural network (CNN) has attracted attention in medical imaging, particularly in its ability to encode high dimensional information in a nonlinear, hierarchical manner. 

Super-resolution~(SR) is a class of techniques that increase the resolution of an imaging system~\cite{SRoverview} and has been widely applied on natural images and is increasingly being explored in medical imaging. Traditional SR methods use linear or non-linear functions (e.g., bilinear/bicubic interpolation and example-based methods~\cite{sparse,sparse1}) to estimate and simulate image distributions. These methods, however, produce blurring and jagged edges in images, which introduce artifacts and may negatively impact the ability of computer-aided detection (CAD) systems to detect subtle nodules. Recently, deep learning, especially convolutional neural networks (CNN), has been shown to extract high-dimensional and non-linear information from images that results in a much improved super-resolution output. One example is the super-resolution convolutional neural network (SRCNN)~\cite{SRCNN}. SRCNN learns an end-to-end mapping from low- to high-resolution images. In~\cite{app1,app2}, the authors applied and evaluated the SRCNN method to improve the image quality of magnified images in chest radiographs and CT images. Moreover,~\cite{ESPCN} introduced an efficient sub-pixel convolution network (ESPCN), which was shown to be more computationally efficient than SRCNN. In~\cite{miccai2017}, the authors proposed a SR method that utilizes a generative adversarial network (GAN), resulting in images have better perceptual quality compared to SRCNN. 
All these methods were evaluated using 2D images. However, for medical imaging modalities that are volumetric, such as CT, a 2D convolution ignores the correlation between slices. We propose a 3DECNN architecture, which executes a series of 3D convolutions on the volumetric data. We measure performance using two image quality metrics: peak signal-to-noise ratio (PSNR) and structural similarity (SSIM). Our approach achieves significant improvement compared with improved SRCNN approach~(FSRCNN)~\cite{FSRCNN} and~\cite{ESPCN} on both metrics.

%We demonstrate that taking use of positional correlations between CT slices are critical to extract image features and generate super resolution images. 

% 1) Unlike existing state-of-art methods which only utilize 2D information, this is the first novel 3D convolutional neural network architecture for image enhancement and super resolution by learning representation from correlated pixels in 3D space; 2) this model has been trained and evaluated using 20672 CT slices from 100 scans of LIDC dataset, and achieves significant improvement compared to existing state-of-art deep learning methods in measurements of both peak signal-to-noise ratio (mean improvement of $0.43 dB$ and $p-value < 2.2e-16$) and structure similarity index (mean improvement of $0.008$ and $p-value < 2.2e-16$). This method can potentially be used to overcome inherent partial volume effects that reduce the accuracy of quantitative measurements. With the same 3DECNN architecture, it also paves the way for other CT image enhancement tasks, such as image denoising and generating high-dose-like CT from low-dose scans.
%for image super-resolution (3DSR-CNN), which makes use of positional correlations between CT slices. The network learns an end-to-end mapping from LR image to HR image.
%2) We investigate on hyperparameters - input depth \emph{n}, number of layers \emph{l}, number of filters \emph{f} and filter size \emph{s} (NLFS), which introduce four sensitive factors to control the convolutional neural network, and also provide a guideline for the design of the neural network.
%3) We demonstrate how the 3D SR-CNN can be applied to address the inherent partial volume effect that reduces the accuracy of quantative measurements (radiomic features) generated from regions of interest. 



% The main contributions of our work are summarized as follows:

% \begin{itemize}

% \item[1)] Different from existing state-of-art methods, we develop the first novel 3D convolutional neural network architecture for CT image enhancement by adaptively learning 3D image representations rather than in 2D. This framework corresponds to the volumetric nature of CT images, overcoming the limitations of existing 2D models.

% \item[2)] The proposed method was trained and evaluated using 20,672 CT slices from 100 scans of the Lung Image Database Consortium (LIDC-IDRI). The model has been compared with several state-of-art deep learning models using PSNR, SSIM and image perceptual quality. Paired t-test is employed to determine the significance of difference in model performance. The results demonstrate that our method achieved significantly better results in both qualitative and quantitative assessments.

% \item[3)] We demonstrate our proposed work by enhancing large slice thickness scans, which can be potentially applied to clinical auxiliary diagnosis of lung cancer. This work also paves the way for other CT image enhancement tasks, such as generating high-dose-like CT from low-dose scans.
% \end{itemize}

==> source files/2_method.tex <==
\section{Method}
\subsection{Overview}

For each slice in the CT volume, our task is to generate a high-resolution image $I^{HR}$ from a low-resolution image $I^{LR}$.
%This problem is ill-posed since we do not have a well-accepted standard to describe what the high resolution image should look like. \hl{Based on the theory of \emph{scale invariance}, the interpolation tuned at the low resolution should be also applicable to the high resolution.}\change{I didn't understand this sentence, rephrase} 
Our approach can be divided into two phases: model training and inference. In the model training phase, we first downsample a given image \emph{I} to obtain the low-resolution image \emph{$I^{LR}$}. We then use the original data as the high-resolution images $I^{HR}$ to train our proposed 3DECNN network. In the model inference phase, we use a previously unseen low-resolution CT volume as input to the trained 3DECNN model and generate a super resolution image $I^{SR}$. 

\begin{figure}[t]
\centering
\includegraphics[height=5.8cm]{./images/fig1_new}
\caption{Proposed 3DECNN architecture}
\label{fig:fig1}
\end{figure}

\subsection{Formulation}
For CT images, spatial correlations exist across three dimensions. As such, the key to generating high-quality SR images is to make full use of available information along all dimensions. Thus, we apply cube-shaped filters on the input CT slices and slides these filters through all three dimensions of the input. Our model architecture is illustrated in Fig. 1. This filtering procedure is repeated in 3 stacked layers. After the 3D filtering process, a 3D deconvolution is used to reconstruct images and up-sample them to larger ones.
%\hl{from the hierarchical information that the previous layer has extracted from the input CT images.}\change{I didn't understand this statement, clarify} 
The output of this 3D deconvolution is a reconstructed SR 3D volume. However, to compare with other SR methods such as SRCNN and ESPCN, which produces 2D outputs, we transform our 3D volume into a 2D output. As such, we add a final convolution layer to smooth pixels into a 2D slice, which is then compared to the outputs of the other methods. In the following paragraphs, we describe mathematical details of our 3DECNN architecture.

%we first apply a \emph{L} layer 3d convolutional neural network directly to the LR image, which arranges its neurons in three dimensions. Every layer of the network transforms the 3D input volume to a 3D output volume of neuron activations.

%Traditional strategy using 2D CNN neural network uses CT slices one by one. This solution ignores the spatial features on the z-dimension. To address this issue, we first apply a \emph{L} layer 3d convolutional neural network directly to the LR image, which arranges its neurons in three dimensions. Every layer of the network transforms the 3D input volume to a 3D output volume of neuron activations.

\subsubsection{3D Convolutional Layers.} 
%\change{your audience will be familiar with this operation, so there is no need to define feature extraction}%Feature extraction means to extract key information in an image. Traditional methods use eigenvectors or singular values of its correlation matrix or frequency signals through Fourier transform~\cite{svd,srembed} to represent image features.
In this work, we incorporate the feature extraction optimizations into the training/learning procedure of convolution kernels. The original CT images are normalized to values between [0,1]. The first CNN layer takes a normalized CT image 
%\change{normalization was not mentioned earlier- clarify how the CT was normalized}, 
(represented as a 3-D tensor) as input and generates multiple 3-D tensors (feature maps) as output by sliding the cube-shaped filters (convolution kernels), which are sized of '$k_1\times k_2\times k_3$', 
%\change{of what size?The filter size discussed in next section} 
across inputs. We define convolution input tensor notations as $\langle N,C_{in},H,W \rangle$ and output $\langle N,C_{out},H,W \rangle$, in which $C_i$ stands for the number of 3-D tensors and  $\langle N,H,W \rangle$ stands for the feature map block's thickness, height, and width, respectively. Subsequent convolution layers take the previous layer's output feature maps as input, which are in a 4-D tensor. Convolution kernels are in a dimension of $\langle C_{in}, C_{out},k_1,k_2,k_3 \rangle$. The sliding stride parameter $\langle s \rangle$ defines how many pixels to skip between each adjacent convolution on input feature maps. Its mathematical expression is written as follows: $ out[c_{o}][n][h][w]=\sum_{n=0}^{C_{i}}\sum_{i=0}^{k_1}\sum_{j=0}^{k_2}\sum_{k=0}^{k_3}W[c_{o}][c_{i}][i][j][k] *In[c_{i}][{s}*n+i][{s}*h+j][{s}*w+k]$.

%\begin{equation}
    %out(N_i, C_{{out}_j}) = \phi(\sum_{k=0}^{C_{in}-1} weight(C_{{out}_j},k) * input(N_i,k) + bias(C_{{out}_j})) .
    %out(N_i, C_{{out}_j}) = \sum_{k=0}^{C_{in}-1} weight(C_{{out}_j},k) * input(N_i,k) + bias(C_{{out}_j}).
%\end{equation}

%\begin{equation}
%\begin{align}
%\begin{split}
    %out(N_i, C_{{out}_j}) = \phi(\sum_{k=0}^{C_{in}-1} weight(C_{{out}_j},k) * input(N_i,k) + bias(C_{{out}_j})) .
%    out[c_{out}][n][h][w]&=\sum_{n=0}^{C_{in}}\sum_{i=0}^{K_1}\sum_{j=0}^{K_2}\sum_{k=0}^{K_3}W[c_{out}][c_{in}][i][j][k]\\
%&\qquad*In[c_{in}][{s}*n+i][{s}*h+j][{s}*w+k].
%\end{equation}
%\end{split}
%\label{equ:conv}
%\end{align}

%where $j \in (1,L)$ is the number of layer. $weight$ is a 3D convolution tensor of size $n_{j-1} \times n_j \times k_j \times k_j \times k_j$, where $n_j$ is the number of features at layer \emph{j}, and $k_j$ is the filter size at layer \emph{j}. $bias$ is represented by a vector of length $C_{{out}_j}$. $\phi$ is the activation function which introduce a non-linear manner. With input size of $(D_{in},H_{in},W_{in})$, the output $(D_{out},H_{out},W_{out})$ can be formulated as:
%\begin{equation}
%\begin{array}{c}
%D_{out} = floor((D_{in}+2*padding[0]-(kernel\_size[0]-1)-1)/stride[0]+1)\\
%H_{out} = floor((H_{in}+2*padding[1]-(kernel\_size[1]-1)-1)/stride[1]+1)\\
%W_{out} = floor((W_{in}+2*padding[2]-(kernel\_size[2]-1)-1)/stride[2]+1) 
%\end{array}
%\end{equation}

%where \emph{stride} controls how many pixels the filter jump at a time as sliding around. \emph{padding} controls the amount of zero-paddings for each dimension. For convenience, we make the output size equals to the input size in this process, and we set the \emph{stride} as 1 to achieve a higher precision. Thus, we can get the value of \emph{padding} when \emph{kernel\_size} is determined. %Apparently, \emph{kernel\_size} is a very important hyper-parameter that sensitive to the output. Besides that, \emph{layer\_number} and \emph{filter\_number} are also very important, and we will discuss how these hyperparameter will influence the output in next section.

\subsubsection{Deconvolution layer.} In traditional image processing, a reverse feature extraction procedure is typically used to reconstruct images. Specifically, design functions such as linear interpolation, are used to up-scale images and also average overlapped output patches to generate the final SR image. In this work, we utilize deconvolution to achieve image up-sampling and reconstruct feature information from previous layers' outputs at the same time. Deconvolution can be thought of as a transposed convolution. Deconvolution operations up-sample input feature maps by multiplying each pixel with %\hl{learnable}\change{what makes these cubic filters learnable? do you mean that the kernel size is learned from the training data?}  
cubic filters and summing up overlap outputs of adjacent filters' output~\cite{deconv}. Following the above convolution's mathematic notations, deconvolution is written as the following: $ out[c_{o}][n][h[w]=\sum_{n=0}^{C_{i}}\sum_{i=0}^{k_1}\sum_{j=0}^{k_2}\sum_{k=0}^{k_3}W[c_{o}][c_{i}][i][j][k]*In[c_{i}][\frac{n}{s}+k_1-i][\frac{h}{s}+k_2-j][\frac{w}{s}+k_3-k]$.
Activation functions are used to apply an element-wise non-linear transformation on the convolution or deconvolution output tensors. In this work, we use ReLU as the activation function. 

%{\color{red}{equations to insert}}
%\begin{align}
%\begin{split}
%\begin{equation}
%out(N_i, C_{{out}_j}) = \phi(\sum_{k=0}^{C_{in}-1} weight(C_{{out}_j},k) * input(N_i,k) + bias(C_{{out}_j})) .
%out[c_{o}][n][h[w]&=\sum_{n=0}^{C_{i}}\sum_{i=0}^{k_1}\sum_{j=0}^{k_2}\sum_{k=0}^{k_3}W[c_{o}][c_{i}][i][j][k]\\
%&\qquad*In[c_{i}][\frac{n}{s}+k_1-i][\frac{h}{s}+k_2-j][\frac{w}{s}+k_3-k].
%\end{equation}
%\end{split}
%\end{align}


%\cite{deconv} Deconvolution layer is often used for reversing the effects of convolution process on max-pooling or other image down-sampling layers. The transposed convolution operator multiplies each input value element-wise by a trainable kernel, and sums over the outputs from all input feature planes. Given a scale factor \emph{k}, we can set the \emph{stride} to k, and deliberately design the \emph{padding} and \emph{kernel\_size} to get a reconstructed HR image that exactly matching the desired HR image size.

%\subsubsection{Feature normalization.} {\color{red} {(Not sure what are you trying to talk about here)}}Without loss of generality, we first consider the algorithm implemented to scale up a image by a factor of three in both \emph{x} and \emph{y} dimension, as in\cite{ESPCN}and\cite{FSRCNN}. To better evaluate how 3D feature extraction influence the final output and compare with traditional 2D CNN flow, we add an additional convolutional layer to reduce the output dimension. We believe that the reconstructed 2D image still cover the information on 3 dimensions. Basically, the behavior of this layer follow up to equation (1), and we can set a full size filter on dimension \emph{z} to reduce this dimension to 1. (need revise)

%\subsection{Activation function}
%{\color{red} {(you do not need a separate section to talk about only the activation function)}}
%Except for the last convolution layer, we add an activation function after each convolution and deconvolution layer. The activation function in neural networks is usually an abstraction representing the probability of firing an action. In this image-to-image application, we treat it as an non-linear transformation from one image to another, as image is an continues non-linear 2D signal. We tested for different activation functions, like sigmoid, relu, tanh. And we found that 'relu' performs better than the others.

% Per the comment above, do not need a separate section to talk about only the activation function
%\subsubsection{Activation function.} Activation functions are used to apply an element-wise non-linear transformation on the convolution or deconvolution output tensors. This function imparts the model with more expressive power. In this work, we use ReLU as the activation function. %It provides our 3DECNN with the ability \hl{to represent non-linear mappings in image transformations. We choose ReLU functions with experiment support}\change{this statement does not make sense to me, clarify}.

\subsubsection{Hyperparameters.}
There are four hyperparameters that have an influence on model performance: number of feature layers, feature map depth, number of convolution kernels, and size of kernels. The number of feature extraction layers $\langle l \rangle$ determines the upper-bound complexity in features that the CNN can learn from images. The feature map depth $\langle n \rangle$ is the number of CT slices that are taken in together to generate one SR image. 
%A small $\langle n \rangle$ provides insufficient info to 3DECNN, but a large $\langle n \rangle$ introduces noisy pixels from the z-dimension. 
The number of convolution kernels $\langle f \rangle$ decides the number of total feature maps in a layer and thus decides the maximum information that can be represented in the output of this layer. The size of convolution and deconvolution kernels $\langle k \rangle$ decides the visible scope that the filter can see in the input CT image or feature maps. 
%A small $\langle k \rangle$ loses local feature information, and a large $\langle k \rangle$ introduces irrelevant adjacent features into account. 
Given the impact of each hyperparameter, we performed a grid search of the hyperparameter space to find the best combination of $\langle n,~l,~f,~k \rangle$ for our 3DECNN model.

%\begin{equation}
%J(w,b) = \frac{1}{m}\sum_{i=1}^{m}L(\hat{y}^{(i)},y^{(i)}) = 
%\frac{1}{m}\sum_{i=1}^{m}||\hat{y}^{(i)}-y^{(i)}||^2
%\end{equation}

\subsubsection{Loss function.}
%The overall objective of SR is to learn an accurate mapping between the low- and high-resolution images that can then be used to enhance lower-resolution images. 
Peak signal-to-noise ratio (PSNR) is the most commonly used metric to measure the quality of reconstructed lossy images in all kinds of imaging systems. A higher PSNR generally indicates a higher quality of the reconstruction image. %PSNR is defined as the log on the division of the max pixel value over mean squared root. The PSNR equation perfectly matches the L2 regularization, a frequently used loss function in deep learning. Therefore, we set L2 regularization as our loss function formulated as below:
PSNR is defined as the log on the division of the max pixel value over mean squared root. Therefore, we directly use the squared mean error function as our loss function: $J(w,b) = \frac{1}{m}\sum_{i=1}^{m}L(\hat{y}^{(i)},y^{(i)}) = \frac{1}{m}\sum_{i=1}^{m}||\hat{y}^{(i)}-y^{(i)}||^2$, where $w$ and $b$ represent \emph{weight} parameters and \emph{bias} parameters. $m$ is the number of training samples. $\hat{y}$ and $y$ refer to the output of the neural network and the target, respectively. In addition, the target loss function is minimized using stochastic gradient descent with the back-propagation algorithm~\cite{backpro}. %The \emph{weight} and \emph{bias} matrices are updated with the following equations:
%\begin{equation}
%\begin{array}{c}
%w:=w-\alpha\frac{\partial J(w,b)}{\partial w},~b:=b-\alpha\frac{\partial J(w,b)}{\partial b}
%\end{array}
%\end{equation}
%where $\alpha$ is the learning rate and $\frac{\partial J(w,b)}{\partial w}$ is the derivative. The \emph{weight} and \emph{bias} are initialized randomly from a Gaussian distribution.



==> source files/3_exp.tex <==
\section{Experiments and Results}

In this section, we first introduce the experiment setup, including dataset and data preparation. Then we show the design space of the hyper-parameters, at which time we show how to explore different CNN architectures and find the best model. Subsequently, we compare our method with recent state-of-the-art work and demonstrate the performance improvement. Lastly, we present examples of the generated SR CT images using our proposed method and previous state-of-the-art results. %to demonstrate the clinical importance of this design, we realize this model to enhance the resolution on Z-direction to overcome inherent partial volume effect that reduce the accuracy of quantative measurements.  
\begin{figure}[t] 
  \centering 
  \subfigure[Influence of feature map depth]{ 
    \label{fig:subfig:a} %% label for first subfigure 
    \includegraphics[width=0.48\linewidth]{./images/fig2a}} 
  %\hspace{1in} 
  \subfigure[Infulence of the number of layers]{ 
    \label{fig:subfig:b} %% label for second subfigure 
    \includegraphics[width=0.48\linewidth]{./images/fig2b}} 
  \subfigure[Influence of the number of kernels]{ 
    \label{fig:subfig:c} %% label for second subfigure 
    \includegraphics[width=0.48\linewidth]{./images/fig2c}} 
  \subfigure[Influence of convolutional kernel size]{ 
    \label{fig:subfig:d} %% label for second subfigure 
    \includegraphics[width=0.48\linewidth]{./images/fig2d}} 
  \caption{Design space of hyper-parameters} 
  \label{fig:1} %% label for entire figure 
\end{figure}

%\begin{figure}[t]
%\subfigure[name of the subfigure]{ 
%\begin{minipage}{0.3\linewidth}
%\includegraphics[]{./images/fig2a} 
%\end{minipage}
%}
%\subfigure[name of the subfigure]{ 
%\begin{minipage}{0.3\linewidth}
%\includegraphics[]{./images/fig2b} 
%\end{minipage}
%}
%\subfigure[name of the subfigure]{ 
%\begin{minipage}{0.3\linewidth} 
%\includegraphics[]{./images/fig2c} 
%\end{minipage}
%}
%\caption{name of the figure} 
%\label{fig:1} 
%\end{figure}

\subsection{Experiment setup}
\subsubsection{Dataset.}
We use the public available Lung Image Database Consortium image collection (LIDC) dataset for this study~\cite{LIDC_2011}, which consists of low- and diagnostic-dose thoracic CT scans. These scans have a wide range of slice thickness ranging from $0.6$ to $5$ $mm$. And the pixel spacing in axial view (x-y direction) ranges from $0.4609$ to $0.9766$ $mm$. We randomly select 100 scans out of a total of 1018 cases from the LIDC dataset, result in a total consisting of 20672 slices. The selected CT scans are then randomized into four folds with similar size. Two folds are used for training, and the remaining two folds are used for validation and test, respectively.


\subsubsection{Data preprocessing.}
%{\color{red}{this paragraph is really cofusing. I don't understnd how you cut images from reading  following paragraph 1 and paragraph 2.}} %We randomly choose 40 scans of 0.75mm thickness for training and 20 scans of 1mm thickness for both validation and test set.
%Each CT 3D scan is first normalized to Hounsfield unit (HU), and then divided into small cube with size of $n*60*60$, where \emph{n} is the sensitive factor defined indicating the correlation of slices (discussed in the next subsection). As mentioned above, we first consider the scaling factor of 3 on both x and y axis. Consequently, bicubic interpolation is used to resize the $n*60*60$ volume to an $n*20*20$ volume as the input LR image.
%We follow the methodology used in~\cite{FSRCNN}. 
For each CT scan, we first downsample it on axial view by the desired scaling factor (set 3 in our experiment) to form the LR images. Then the corresponding HR images are ground truth images.
%Then we crop the LR training images into a set of $m\times m$-pixel sub-images with a stride $m$(set 20 in our experiment). 
%Also  sub-images (with size $3m\times 3m$) are also cropped from the ground truth images.


\subsubsection{Hyperparameter tuning $\langle n,~l,~f,~k \rangle$.}
We choose the four most influential parameters to explore in our experiment and discuss, which is \emph{feature depth (n)}, \emph{number of layers (l)}, \emph{number of filters (f)} and \emph{filter kernel size (k)}.% We design a set of controlling (very chineglish...) experiments with different values of these parameters.

The effect of the \textbf{feature depth $\langle n\rangle$} is shown in Fig.~\ref{fig:subfig:a}. It presents the training curves of three different 3DECNN architectures, in which their $\langle l,~f,~s \rangle$ are the same and $\langle n \rangle$ varies in $[3,~5,~9]$. Among the three configurations, $n=3$ has a better average PSNR than the others.
%a slightly better average PSNR than $n=5$ and a bit more better PSNR than $n=9$. 
The effect of the \textbf{number of layers $\langle l \rangle$} is shown Fig.~\ref{fig:subfig:b}, which demonstrates that a deeper CNN may not always be better. With fixed $\langle n,~f,~s \rangle$ and varying $l \in [1,3,5,8]$, here $l$ indicate the number of convolutional layers before the deconvolution process. we can observe apparent different performance on the training curves. We determine that $l=3$ achieves higher average PSNR.
%the goal of minimizing the average PSNR.
%\change{do you mean PSNR?}.
The effect of the \textbf{number of filters $\langle f \rangle$} is shown in Fig.~\ref{fig:subfig:c}, in which we fix $\langle n,~l,~k \rangle$ and choose $\langle f \rangle$ in four collections.
%the following collection $\langle 16,~16,~16,~32,~1 \rangle$, $\langle 32,~32,~32,~32,~1 \rangle$, $\langle 64,~64,~64,~32,~1 \rangle$ and $\langle 64,~64,~32,~32,~1 \rangle$. 
An apparent drop in PSNR is seen when $\langle f \rangle$ chooses the too small configuration $\langle 16,~16,~16,~32,~1 \rangle$. $\langle 64,~64,~64,~32,~1 \rangle$ and $\langle 64,~64,~32,~32,~1 \rangle$ has approximately the same PSNR (28.66 vs. 28.67) so we choose latter one to save training time. 
The effect of the \textbf{filter kernel size $\langle k \rangle$} is shown in Fig.~\ref{fig:subfig:d}, in which we fix $\langle n,~l,~f \rangle$ and vary k in the collection of $[3,~5,~9]$. Experiment result proves that $k=3$ achieves the best PSNR. The PSNR decrease with filter kernel size demonstrate that relatively remote pixels contribute less to feature extraction and bring much signal noise to the final result.
%\subsubsection{Proper feature map thickness: $\langle n\rangle$.} . Thus the input depth \emph{n} is sensitive, and we take a set of experiments with varying \emph{n}. From the experimental results shown as Fig.\ref{fig:subfig:a}, it achieves peak performance at $n=5$. 

%\subsubsection{Deeper may not be the better: $\langle l \rangle$.} 
%Specifically, we test the performance with different layer numbers in the 3D feature extraction stage. As illustrated on Fig. \ref{fig:subfig:b}, the number of layers \emph{l} varies from 1 to 8 with fixed \emph{f} and \emph{s}. We can see from the experiment that it is not "the deeper the better; there is even a little drop when \emph{l} reaches 8.

%\subsubsection{More filters extract more features: $\langle f \rangle$.}
%In this experiment, both \emph{l} and \emph{s} are fixed and \emph{f} varies from 16 to 64. As shown in Fig. \ref{fig:subfig:c}, we find that more filters could achieve better performance. At the same the complexity and the training time will increase with filter numbers. Therefore, this is a trade-off between performance and complexity.

%\subsubsection{Choose moderate filter size: $\langle k \rangle$.} 
%The last set of experiments treat `$k$' as variable, and we can see from Fig. \ref{fig:subfig:d} that a large filter size may lead to bad results. We can also explain it from the perspective of \emph{correlation}---that is, the correlation of pixels will become weaker and weaker with the distance increasing. 

\subsubsection{Final model.}
%\emph{l} = 3, $(f_1,s_1)=64,5$, $(f_2,s_2)=32,3$, $(f_3,s_3)=32,3$. On the feature normalization layer, we set $(f,s)=32,3$ and on the deconvolution layer, we set $(f,s)=1,5$.
For the final design, we set $\langle~ n, l, (f_1,k_1),(f_2,k_2),(f_3,k_3),(f_4^{deconv},\\k_4^{deconv}),(f_5,k_5) ~\rangle$ 
$ = \langle 5, 3,(64,3),(64,3), (32,3),(32,3),(1,3) \rangle$. We set the learning rate $\alpha$ as $10^{-3}$ for this design and achieve a good convergence. We implemented our 3DECNN model using Pytorch and trained/validated our model on a workstation with a NVIDIA Tesla K40 GPU. The training process took roughly 10 hours. 
%on \hl{42000}\change{This number is different from what was stated earlier (20,672 CT slices). How the 42,000 training samples were obtained should be clarified.} training samples. %Fig. 3 shows the feature maps of the first three convolutional layers in the training process.
\begin{table}[t]
\centering
\caption{PSNR and SSIM results comparison.}
\includegraphics[height=3cm]{./images/table1_new}
\label{table:table1}
\end{table}
% \begin{figure}[t]
% \centering
% \includegraphics[height=5cm]{./images/fig3}
% \caption{Features of the first three layers}
% \label{fig:fig4}
% \end{figure}


% \begin{figure}[t]
% \centering
% \begin{minipage}[t]{0.8\textwidth}
% \centering
% \includegraphics[width=9cm]{./images/fig3_new.png}
% \caption{Comparison with the-state-of-the-art works}
% \label{fig:fig3}
% \end{minipage}
% \centering
% \begin{minipage}[t]{0.8\textwidth}
% \centering
% \caption{PSNR and SSIM results comparison.}
% \begin{table}
% \includegraphics[width=10cm]{./images/table1.png}
% \label{table:table1}
% \end{table}
% \end{minipage}
% \end{figure}



%\begin{figure}[t]
%\centering
%\includegraphics[height=9cm]{./images/fig3_new.png}
%\caption{Comparison with the-state-of-the-art works}
%\todo[inline]{Make the original image the same size as the resized image- the benefit of SR for the medical image community is not that we can generate images with larger dimensions, but rather, the sharpness and detail of the images are improved.}
%\label{fig:fig3}
%\end{figure}

%\begin{table}[h]
%\centering
%\caption{PSNR and SSIM results comparison.}
%\includegraphics[height=3cm]{./images/table1}
%\label{table:table1}
%\end{table}

% \begin{figure}[t]
% \centering
% \includegraphics[height=15cm]{./images/fig5.png}
% \caption{Performance visualization of enhancing large thickness scan on axial, sagittal, and coronal axis}
% \label{fig:fig5}
% \end{figure}

\subsection{Results comparison with T-test validation}
% This is already stated in the Methods section: To objectively measure the model performance, PSNR and SSIM are both employed as the quantitative metrics. PSNR quantifies the mean pixel intensity differences between the model output and original image (ground truth). SSIM access the perceived image quality in objective way.
We compare the proposed model to bicubic interpolation and two existing the-state-of-the-art deep learning methods for super resolution image enhancement: 1) FSRCNN~\cite{FSRCNN} and 2) ESPCN~\cite{ESPCN}. We reimplemented both methods, retraining and testing them in the manner as our proposed method. Both the FSRCNN-s and the FSRCNN architectures used in~\cite{FSRCNN} are compared here. A paired t-test is adopted to determine whether a statistically significant difference exists in mean measurements of PSNR and SSIM when comparing 3DECNN to bicubic, FSRCNN, and ESPCN. Table 1 shows the mean and standard deviation for the four methods in PSNR and SSIM using 5,168 test slices. The paired t-test results show that the proposed method has significantly higher mean PSNR, and mean differences are 2.0183 dB (p-value $< 2.2e-16$), 0.8357 dB (p-value $< 2.2e-16$), 0.5406 dB (p-value $< 2.2e-16$), and 0.4318 dB (p-value $< 2.2e-16$) for bicubic, FSRCNN-s, FSRCNN and ESPCN, respectively. 
It also shows that out model has significantly higher SSIM, and the mean differences are $0.0389$ (p-value $< 2.2e-16$), $0.0136$ (p-value $< 2.2e-16$), $0.0098$ (p-value $< 2.2e-16$), and $0.0080$ (p-value $< 2.2e-16$). 
%All metrics suggest that our approach is significantly better, which demonstrate 3DECNN extract more features from volumetric studies and outperform the comparison 2D approaches.
To subjectively measure the image perceived quality, we also visualize and compare the enhanced images in Fig. \ref{fig:fig3}. The zoomed areas in the figure are lung nodules. As the figures shown, our approach achieved better perceived quality compared to other methods.

\begin{figure}[t]
\centering
\includegraphics[height=8cm]{./images/fig3_new.png}
\caption{Comparison with the-state-of-the-art works}
\label{fig:fig3}
\end{figure}
%More experiment results please refer to the website {\color{red}{are you sure?}}.\footnote{Submit to the supplementary materials as anonymous rule.}

% you fogot to upload fig-5
%\begin{figure}[t]
%\centering
%\includegraphics[height=6.2cm]{./images/fig5}
%\caption{Illustration of 3d-CNN based architecture}
%\label{fig:fig1}
%\end{figure}


%\subsection{Application of enhancing resolution on z-direction}(need revise)
%Medical image enhancement is meaningful in clinical trails, because clear images help doctors more easily to detect disease, like lung cancer. CT images usually has a large slice thickness on z-direction, which need up-sampling. Based on the proposed design, We made a simple modification on deconvolution layer to upscale on one dimension. As shown on Fig.6, the proposed method provide a better visualization than traditional methods.

% \subsection{Performance visualization on enhancing large-slice thickness CT scan}
% CT studies have varying resolutions, particularly in the z-direction, which can hinder tasks such as nodule characterization. In this experiment, we take a high-resolution scan with slice thickness of 1mm. First we generate a 3mm low-resolution scan from the high-resolution scan using bicubic interpolation. Then the proposed method is used to reconstruct the low-resolution scan back to 1mm. As illustrated in Fig. \ref{fig:fig5}, we show the axial, sagittal, and coronal axis alongside the results for bicubic and the proposed approach. Our proposed method shows good perceptual quality and can potentially be used to overcome the inherent partial volume effect.























==> source files/4_conclu.tex <==
\section{Discussion and Future work}
We present the results of our proposed 3DECNN approach to improve the image quality of CT studies that are acquired at varying, lower resolutions. Our method achieves a significant improvement compared to existing state-of-art deep learning methods in PSNR (mean improvement of $0.43 dB$ and p-value $< 2.2e-16$) and SSIM (mean improvement of $0.008$ and p-value $< 2.2e-16$). We demonstrate our proposed work by enhancing large slice thickness scans, which can be potentially applied to clinical auxiliary diagnosis of lung cancer. As future work, we explore how our approach can be extended to perform image normalization and enhancement of ultra low-dose CT images (studies that are acquired at 25\% or 50\% dose compared to current low-dose images) with the goal of producing comparable image quality while reducing radiation exposure to patients.

%Through the provided examples, we demonstrate how our algorithm is capable of overcoming partial volume effect in thick section CT images. As part of future work, we will investigate whether volumetric measurements taken using our 3DECNN approach achieves the same values as those taken using higher resolution scans of the same object compared to thick section scans. We will also apply this work to image enhancement of ultra low-dose CT images with the goal of producing image quality that is comparable to those acquired at higher doses.

==> source files/5_acknowledge.tex <==
\section{Acknowledgement}
This work is partly supported by National Natural Science Foundation of China (NSFC) Grant 61520106004, the National Institutes for Health under award No. R01CA210360. The authors would also like to thank the UCLA/PKU Joint Research Institute, Chinese Scholarship Council for their support of our research.
